Electromagnetic Calorimeter for HADES

We propose to build the Electromagnetic calorimeter for the HADES di-lepton spectrometer. It will enable to measure the data on neutral meson production from nucleus-nucleus collisions, which are essential for interpretation of dilepton data, but are unknown in the energy range of planned experiments (2-10 GeV per nucleon). The calorimeter will improve the electron-hadron separation, and will be used for detection of photons from strange resonances in elementary and HI reactions. Detailed description of the detector layout, the support structure, the electronic readout and its performance studied via Monte Carlo simulations and series of dedicated test experiments is presented. The device will cover the total area of about 8 m^2 at polar angles between 12 and 45 degrees with almost full azimuthal coverage. The photon and electron energy resolution achieved in test experiments amounts to 5-6%/sqrt(E[GeV]) which is sufficient for the eta meson reconstruction with S/B ratio of 0.4% in Ni+Ni collisions at 8 AGeV. A purity of the identified leptons after the hadron rejection, resulting from simulations based on the test measurements, is better than 80% at momenta above 500 MeV/c, where time-of-flight cannot be used.

==> Costs/Costs.tex <==


\section{Cost Estimation}


Estimated components costs [in EURO] are shown in Table \ref{table:tab_costs}: 



\begin{table}[h!]
  \begin{tabular*}{12.0cm}{  c  c  c  c }
    \hline
    \bf{Mechanical Structure} \\ 
    && Total \\ \hline
    Support Construction & & 69.800 \\ \hline
    \bf{PMTs  and HV} \\ 
    & Unit Cost & Total \\ \hline
    Power supply & & 160.000 \\
     Mechanics * & & 40.000 \\
     PMTs & 500 & 150.000(300) \\ \hline 
    \bf{FE  and Digitizing boards} \\ 
&     Unit Cost 	&  Total \\\hline
   front-end board			&	425		&		17850 (42)\\
TRBv3 			&	1500		&		9000 (6)\\
ADC card			&	 1200		&		  7200 (6)\\ \hline
Total  && 453.850 \\ \hline
\end{tabular*}  
\caption{Estimated costs for the HADES EM calorimeter.}
 \label{table:tab_costs}  
\end{table}

\noindent
Comments:

$^{*}$The Mechanics costs includes the modifications to the glass module geometry and the polishing.


As stated in the text, the version of the Calorimeter with higher granularity
of modules at low polar angle region (modules in 2-3 ``lowermost'' rows 
replaced by modules with transverse size 45x45 mm$^2$) is under consideration.
In this case number of channel would increase by up to 300 channels (30\%),
and the costs would increase accordingly.

 
%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> Electronics/Electronics.tex <==
\section{Electronics}
\subsection{Photomultiplier and HV Supply}
\subsection{Front-End Electronics and Read-Out}


==> Electronics/PMT.tex <==
\subsection{Photo Multiplier}



==> Intro/intro_calorimeter.tex <==
\section{Introduction}



Dielepton measurements at SIS100 and SIS300 energy domain are mandatory to established 
a complete excitation function of the virtual photon radiation from dense nuclear 
matter over the whole energy region available at the current HI machines.  
Dielectron results obtained at the lowest SPS energies of $40$ AGeV by CERES collaboration 
demonstrate a large pair excess in the intermediate ($0.14 < M < 0.6 GeV/c^{2}$) mass region 
pointing to a strong source located in the high density zone of HI collisions.
A precise determination of this excess, however, depends on a precise knowledge
of the hadronic cocktail, which for 2-40 AGeV, is dominated 
by the $\eta$ Dalitz decay. Furthermore, a convenient
normalization of the dielectron spectra is naturally given by the
$\pi^0$ yield dominating the low mass region ($0.14 < M$).  These two reasons 
requires data on the inclusive cross sections $\pi^0$ and $\eta$ mesons. 

For the SIS18 energy range, production of neutral
mesons has been studied extensively in HI collisions by the TAPS collaboration via
photon calorimetry and in $N-N$ collisions by various detectors at Upsalla, Saclay and COSY. 
However, for the $8-40$ AGeV range no respective data at all
do presently exist, with the consequence that any interpretation of
future dielectron data would have to depend solely on theoretical
models, e.g. transport calculations or appropriate hydrodynamical
models. In order to remedy this situation we propose to measure the
respective $\pi^0$ and $\eta$ meson yields together with the
dielectron data in $p-p$ and HI collisions. Furthermore, photon measurement 
would be of large interest for the HADES strangeness programme which 
address also spectroscopy of neutral $\Lambda(1405)$ and $\Sigma(1385$ 
resonances in elementary and HI reactions. 


This goals can be achieved by replacing the HADES Pre-Shower detector, located at forward angles
($18^{\circ}<\theta<45^{\circ}$), with an electromagnetic
calorimeter based on lead-glass modules obtained on loan from the OPAL
detector. An additional advantage of such a device would be the better electron/pion suppression that
it offers at large momenta (p$>$400 MeV/c) as compared to the
present situation.  Note that at lower momenta the electron/hadron
identification is provided by the RICH, RPC and TOF detectors already 
available in HADES.

The total are of the proposed HADES calorimeter amounts to about
8\,m$^{2}$ and covers polar angles between $12$ and $45^0$ with almost 
full azimuthal coverage. The photon and electron energy resolution achieved in 
test experiments  amounts to 5\%/$\sqrt{E}$ which is sufficient for the $\eta$ meson
reconstruction with S/B ratio of $\sim\1.5\%$ in $Ni+Ni$ collisions at 8 AGeV. 
The selected granularity of the detector results in $978$ modules (.. to be completed..)
 
Below we present details of the detector layout, electronic readout and its performance 
studied via Monte Carlo Simulations and series of dedicated test experiments.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> People/People.tex <==
\section{Organization}


\begin{table}[h!]
\begin{tabular*}{12.0cm}{  c  c  c }
\hline
  {\bf subproject}   & {\bf coordinator} & {\bf teams}    \\   \hline \hline
  mechanics        & E. Lisowski & Uni. Krakow            \\ \hline
  detector modules & F. Guber    & INP Moscow, NPI Rez    \\  \hline 
  electronics      & M. Traxler  & Uni. Krakow, GSI       \\  \hline
  simulations      & K. Lapidus  & TU Munich              \\  \hline
  tests            & P. Tlusty   & NPI Rez, INP Moscow, Uni. Frankfurt \\  \hline


\end{tabular*}  
\caption{List of subprojects, coordinators and involved teams.}
 \label{table:people}  
\end{table}


==> Simulation/occupancy_section.tex <==
\subsection{Occupancy considerations}

The occupancy of the calorimeter modules was studied with simulations taking as an input $^{56}${Ni}+$^{56}$Ni collisions at 8~AGeV with a centrality selection corresponding to $b<1$~fm. The events have been generated with the UrQMD transport code. The choice of the collision system and the impact parameter range ensures the highest possible multiplicity conditions to be studied with the HADES set-up.  

Fig.~\ref{fig:occupancy_15} (left) illustrates the event-averaged calorimeter cells occupancy. A cut on the minimal energy deposition of 15 MeV was applied. Squares correspond to the centers of the calorimeter modules. In the investigated conditions the highest occupancy of 80\% ??? is observed for the modules in the two innermost rows. 

In order to cope with the high occupancy at low polar angles, a high-granularity version of the calorimeter geometry was considered in which the lead-glass crystals in the two innermost rows have lateral dimension that is one fourth of the usual crystal size. The right panel of Fig.~\ref{fig:occupancy_15} illustrates the occupancy for the high-granularity version. In this case the maximal occupancy drops to 40\% for the small modules.

It should be stressed that the high occupancy of the cells is caused mainly by the particles with low energy deposition (hadrons) and does not necessarily obstruct realization of the main objectives: the electron/pion separation at high values of particle momenta and neutral meson reconstruction. It drops rather quickly with the rise of the energy cut: taking into account cells with minimal energy deposition of 100 MeV, the highest occupancy (in the standard geometry) does not exceed value of 45\%.

\begin{figure}[htbp] %  figure placement: here, top, bottom, or page
   \centering
   \includegraphics[width=15cm]{occupancy_NiNi_8_1fm_15MeV.eps} 
   \caption{Average module occupancy in Ni~+~Ni collisions at 8~AGeV beam kinetic energy and impact parameter $b < 1$~fm for the standard (left) and increased granularity (right) calorimeter setup}
   \label{fig:occupancy_15}
\end{figure}

In the following, results for the electron-pion separation and reconstruction of neutral mesons will be presented, as obtained in the standard version of the calorimeter geometry.
